Pirates of Charity: Exploring Donation-based Abuses in Social Media Platforms

With the widespread use of social media, organizations, and individuals use these platforms to raise funds and support causes. Unfortunately, this has led to the rise of scammers in soliciting fraudulent donations. In this study, we conduct a large-scale analysis of donation-based scams on social media platforms. More specifically, we studied profile creation and scam operation fraudulent donation solicitation on X, Instagram, Facebook, YouTube, and Telegram. By collecting data from 151,966 accounts and their 3,053,333 posts related to donations between March 2024 and May 2024, we identified 832 scammers using various techniques to deceive users into making fraudulent donations. Analyzing the fraud communication channels such as phone number, email, and external URL linked, we show that these scamming accounts perform various fraudulent donation schemes, including classic abuse such as fake fundraising website setup, crowdsourcing fundraising, and asking users to communicate via email, phone, and pay via various payment methods. Through collaboration with industry partners PayPal and cryptocurrency abuse database Chainabuse, we further validated the scams and measured the financial losses on these platforms. Our study highlights significant weaknesses in social media platforms' ability to protect users from fraudulent donations. Additionally, we recommended social media platforms, and financial services for taking proactive steps to block these fraudulent activities. Our study provides a foundation for the security community and researchers to automate detecting and mitigating fraudulent donation solicitation on social media platforms.

==> profile_posts_image_sentiments_analysis.tex <==
\begin{figure*}[t!]
    \centering
    \subcaptionbox{Scammer Interactions.\label{fig:si_at}}{\includegraphics[width=0.31\textwidth]{images/posts_graph.pdf}}\hfill
    \subcaptionbox{Following Count.\label{fig:si_ap}}{\includegraphics[width=0.30\textwidth]{images/followers_graph.pdf}}\hfill
    \subcaptionbox{Profile Creation Date.\label{fig:si_ac}}{\includegraphics[width=0.35\textwidth]{images/account_create_date.pdf}}

    \caption{Engagment and age of scammer profile from each of the social media platforms -- \autoref{fig:si_at} shows the engagement of scammer via posts, \autoref{fig:si_ap} shows the {\em following} count of scammers and \autoref{fig:si_ac} shows the age of scammers based on profile creation date from each of the social media platforms that we studied.}
    \label{fig:scammer_profile_evaluation}
\end{figure*}

\section{Anatomy of Scam Accounts and Engagement}
\label{sec:scammer_profile_posts_image_comment}

In this section, we explore the creation and engagement tactics of scammers involved in fraudulent donation schemes. Specifically, we examine three key aspects: (i) how scammers represent themselves through profile metadata (\autoref{sec:profile_content_and_association}), (iii) the clustering of posts to detect coordinated attacks during engagement (\autoref{sec:post-clustering}). Additionally, we provide scam operation and network analysis in \autoref{sec:scam_network analysis}. Through this analysis, we provide a comprehensive study of scammers' profile creation, engagement strategies, and operation beyond the point of scam origin. 

\input{posts_clustering}
